Communicating Is Crowdsourcing: Wi-Fi Indoor Localization with CSI-based Speed Estimation

Numerous indoor localization techniques have been proposed recently to meet the intensive demand for location based service, and Wi-Fi fingerprint-based approaches are the most popular and inexpensive solutions. Among them, one of the main trends is to incorporate the built-in sensors of smartphone and to exploit crowdsourcing potentials. However the noisy built-in sensors and multi-tasking limitation of underline OS often hinder the effectiveness of these schemes. In this work, we propose a passive crowdsourcing CSI-based indoor localization scheme, C2 IL. Our scheme C2 IL only requires the locating-device (e.g., a phone) to have a 802.11n wireless connection, and it does not rely on inertial sensors only existing in some smartphones. C2 IL is built upon our innovative method to accurately estimate the moving distance purely based on 802.11n Channel State Information (CSI). Our extensive evaluations show that the moving distance estimation error of our scheme is within 3% of the actual moving distance regardless of varying speeds and environment. Relying on the accurate moving distance estimation as constraints, we are able to construct a more accurate mapping between RSS fingerprints and location. To address the challenges of collecting fingerprints, a crowdsourcing- based scheme is designed to gradually establish the mapping and populate the fingerprints. In C2 IL, we design a trajectory clustering-based localization algorithm to provide precise real-time indoor localization and tracking. We developed and deployed a practical working system of C2 IL in a large office environment. Extensive evaluation results indicate that our scheme C2 IL provides accurate localization with error 2m at 80% at very complex indoor environment with minimal overhead.

==> mobi-overview.tex <==
To minimizing the 
Since CSI and RSS can be estimated by both APs and clients,
\ourprotocol  can be deployed in either AP-end or client-end. 
Whenever it is deployed at either end, the core of the system remains
 same.  
In the rest of the paper, for simplicity of presentation, we assume
 that WiFi APs will collect the  signal and conduct the needed
 computation. 
The positions of WiFi APs are not required to be known in either case.


\begin{figure}[tb]
\begin{center}
\includegraphics[scale=0.5]{figures/overview2.pdf}
\end{center}
\vspace{-0.25in}
\caption{\ourprotocol  System Architecture.}
\vspace{-0.1in}
\label{fig:overview1}
\end{figure}

Fig.~\ref{fig:overview1} demonstrates our system architecture.
When a user enters the building, we assume that the device held by the
 user will build wireless connections with the APs inside the building.
The IEEE 802.11n WiFi APs will record the RSS values and the CSI
 values of the received  signal from the client device and send the
 data to a localization  server.
Based on the sequence of the CSI values taken during a time-window,
 the server  will  then quickly estimate the moving distance of the
 client in this  time-window.
The RSS values will be used to build a matching with the fingerprint
 RSS values  stored in the fingerprint database, which itself is
 populated using crowdsourcing techniques.
The estimated moving distance, together with the estimated geodesic distance of
different fingerprint locations  in the map, will be used to further improve the
quality of the matching, and thus, the accuracy of the localization.
In the rest we discuss in detail each of the components in \ourprotocol.









